ChatGPT as a Math Questioner? Evaluating ChatGPT on Generating Pre-university Math Questions

Mathematical questioning is crucial for assessing students problem-solving skills. Since manually creating such questions requires substantial effort, automatic methods have been explored. Existing state-of-the-art models rely on fine-tuning strategies and struggle to generate questions that heavily involve multiple steps of logical and arithmetic reasoning. Meanwhile, large language models(LLMs) such as ChatGPT have excelled in many NLP tasks involving logical and arithmetic reasoning. Nonetheless, their applications in generating educational questions are underutilized, especially in the field of mathematics. To bridge this gap, we take the first step to conduct an in-depth analysis of ChatGPT in generating pre-university math questions. Our analysis is categorized into two main settings: context-aware and context-unaware. In the context-aware setting, we evaluate ChatGPT on existing math question-answering benchmarks covering elementary, secondary, and ternary classes. In the context-unaware setting, we evaluate ChatGPT in generating math questions for each lesson from pre-university math curriculums that we crawl. Our crawling results in TopicMath, a comprehensive and novel collection of pre-university math curriculums collected from 121 math topics and 428 lessons from elementary, secondary, and tertiary classes. Through this analysis, we aim to provide insight into the potential of ChatGPT as a math questioner.

==> basepromptaware.tex <==
\begin{tcolorbox}[
    colback=gray!20, % Background color of the box
    colframe=gray!50, % Border color of the box
    arc=4mm, % Curved corner radius
    title=Base prompt for answer-aware,
    coltitle=black]
Your task is to generate a math question, given its answer and a piece of context. Given the following context which is delimited with triple backticks:```[\textcolor{blue}{context}]```. The expected answer is: [\textcolor{blue}{solution}].\\
Avoid incorporating contextual information into the generated question since the generated question will be appended after the context to make a complete math problem.  \\
Ensure that the tense of the generated question matches that of the context. \\
 The generated question should have below 20 words.
\\The question is:
% \end{tcbraster}
\label{base-prompt-aware}
\end{tcolorbox}

==> basepromptcontextunaware.tex <==
% \begin{tcolorbox}[

%     colback=gray!20, % Background color of the box
%     colframe=gray!50, % Border color of the box
%     arc=4mm, % Curved corner radius
%     title=Base prompt for answer-unaware-high school,
%     coltitle=black]
% % \end{tcbraster}
%             Define Difficulty Level is: \\
%             1: The difficulty of the generated question is appropriate for students at the lower elementary school level. \\
%             2: The difficulty of the generated question is appropriate for students at the upper elementary school level. \\
%             3: The difficulty of the generated question is appropriate for students at the middle school level. \\
%             4: The difficulty of the generated question is appropriate for students at the high school level. \\
%             5: The difficulty of the generated question is appropriate for Mathematics contests such as IMO, or marked as \emph{challenging problem} (10th grade - 12th grade, follow Khan Academy)\\

%             Define the [\textcolor{blue}{subtopic name}] topic as: [\textcolor{blue}{subtopic definition}]. Generate a math problem with its answer at Difficulty Level [\textcolor{blue}{difficulty}] in the topic of [\textcolor{blue}{topic}]: [\textcolor{blue}{subtopic name}]. 
            
%             Your questions are required to be diverse in terms of tokens, which can be achieved by paraphrasing the question or introducing/renaming variables, ...
            
%             You are also given a demonstration:
%             [\textcolor{blue}{prompt demonstration}]
            
%             Your response should follow the format: Question: [your generated question]$\backslash$nAnswer:{{answer to the question}}'''


% \label{base-prompt}
% \end{tcolorbox}

% \begin{tcolorbox}[
%     colback=gray!20, % Background color of the box
%     colframe=gray!50, % Border color of the box
%     arc=4mm, % Curved corner radius
%     title=Base prompt for answer-unaware-grade 1-8,
%     coltitle=black]
% % \end{tcbraster}
%             Define Difficulty Level is: \\
%             1: The difficulty of the generated question is appropriate for students at the lower elementary school level. \\
%             2: The difficulty of the generated question is appropriate for students at the upper elementary school level. \\
%             3: The difficulty of the generated question is appropriate for students at the middle school level. \\
%             4: The difficulty of the generated question is appropriate for students at the high school level. \\
%             5: The difficulty of the generated question is appropriate for Mathematics contests such as IMO, or marked as \emph{challenging problem} (10th grade - 12th grade, follow Khan Academy) \\

%             Define the [\textcolor{blue}{subtopic name}] topic as: [\textcolor{blue}{subtopic definition}]. Generate a math problem with its answer at Difficulty Level [\textcolor{blue}{difficulty}] in the topic of [\textcolor{blue}{topic}]: [\textcolor{blue}{subtopic name}]. \\

%             You could introduce characters, objects, or scenarios to make your math problem context more diverse in terms of tokens. \\
%             You should show your chain of thought that leads to the final answer in the solution, but keep it concise. \\
            
%             You are also given a demonstration:
%             [\textcolor{blue}{prompt demonstration}]
            
%             Your response should follow the format: Question: [your generated question]$\backslash$nAnswer:{{answer to the question}}'''


% \label{base-prompt}
% \end{tcolorbox}

==> basepromptunaware.tex <==
\begin{tcolorbox}[
    colback=gray!20, % Background color of the box
    colframe=gray!50, % Border color of the box
    arc=4mm, % Curved corner radius
    title=Base prompt for answer-unaware,
    coltitle=black]
Your task is to generate a math question, given a piece of context. Given the following context which is delimited with triple backticks:```[\textcolor{blue}{context}]```.\\ 
Avoid incorporating contextual information into the generated question since the generated question will be appended after the context to make a complete math problem.  \\
Ensure that the tense of the generated question matches that of the context. \\
 The generated question should have below 20 words.
\\The question is:
% \end{tcbraster}
\label{base-prompt}
\end{tcolorbox}

==> diffdistpreumath.tex <==
% \setlength{\tabcolsep}{3.5pt}
% \renewcommand{\arraystretch}{1.25} 
% \begin{table}[h]
% \scriptsize
% % \setlength{\extrarowheight}{5pt}
% \begin{tabular}{cccccccccc}

% \cline{1-9}

% \multirow{2}{*}{\textbf{Class}} & \multirow{2}{*}{\textbf{\#topics}} & \multirow{2}{*}{\textbf{\#subtopics}} &  \multirow{2}{*}{{\makecell{\textbf{\#QA}\\ \textbf{pairs}}}} & 
% % \makecell{\textbf{Difficulty}\\ \textbf{distribution}} 
% \multicolumn{5}{c}{\textbf{Difficulty distribution}}\\ 
% \multicolumn{4}{c}{} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5}\\
% \cline{1-9}
% Grade 1 & 2 & 4 & 61 & 61 & 0 & 0 & 0 & 0        \\
% Grade 2 & 6 & 24 & 327 &  327  & 0 & 0 & 0 & 0   \\
% Grade 3 & 11 & 36 & 506 & 506 & 0 & 0 & 0 & 0     \\
% Grade 4 & 11 & 20 & 350 & 0 & 350   & 0 & 0 & 0  \\
% Grade 5 & 15 & 30 & 558 & 0 & 558  & 0 & 0 & 0    \\
% Grade 6 & 11 & 30 & 1165 & 0 & 0 & 1165 & 0 & 0 \\
% Grade 7 & 7 & 23 & 853 & 0 & 0 & 853 & 0 & 0\\
% Grade 8 & 7 & 32 & 1231 & 0 & 0 & 1231 & 0 & 0\\
%  \makecell{High\\ school} & 51 & 229 & 11032 & 0 & 0 &  60 & 8796& 2176\\
% \cline{1-9}
% Total & 121 & 428 & 16083 &  894 & 908 & 3309 & 8796 & 2176 \\ 
% \cline{1-9} \\

% \end{tabular}
% \vspace{-3mm}
% \caption{Difficulty distribution of PRE-UMATH by grades.} \label{tab:diffdist}
% \label{table2}
% \end{table}
% % \vspace{-10mm}

==> editchatgpt.tex <==
\begin{table*}[]
\section{Dataset Post-editing}
\label{daposedit}    
    
    \small
    \centering
    \begin{tabular}{c}
        \includegraphics[width=0.7\textwidth]{imgs/khan_1.png} \\
        \begin{minipage}[t]{0.8\textwidth}
\textcolor{blue}{Question}: What is the greatest common factor of $30b^2$, $80b^2$, and $20b^3$?

\textcolor{blue}{Edited ChatGPT's answer}:Let's analyze each term individually: $30b^2$ can be factored as $2\times3\times5\times b^2$. $80b^2$ can be factored as $2^4\times5\times b^2.$ $20b^3$ can be factored as $2^2\times5\times b^3$.To find the GCF, we look for the common factors with the lowest exponent. Looking at the prime factors, we can see that the highest power of b that divides all three terms is $b^2$. Additionally, the largest numerical factor that divides the coefficients is \textcolor{red}{\st{2}} \textcolor{green}{10}. Therefore, the greatest common factor of $30b^2$, $80b^2$, and $20b^3$ is \textcolor{red}{\st{$2b^2$}} \textcolor{green}{$10b^2$}.

% \textcolor{blue}{Edit rate:} 3\%
        \end{minipage} \\

    \end{tabular}

\vspace{10pt}
\begin{tabular}{c}
        \includegraphics[width=0.7\textwidth]{imgs/khan_2.png} \\
        \begin{minipage}[t]{0.8\textwidth}

        
\textcolor{blue}{Question}: What is the value of x in the figure shown below:$\backslash$nBEGIN PLOT:$\backslash$nDraw( ABCD)$\backslash$nLabel(Angle CBA, 88 $\backslash$degree) $\backslash$nLabel(Angle ACB, 53 $\backslash$degree) $\backslash$nLabel(Angle CBD, x $\backslash$degree) $\backslash$nLabel(Length CD, 4.5)$\backslash$nLabel(Length BD, 5.6)$\backslash$nLabel(Length AC, 5.6)$\backslash$nLabel(Length AB, 4.5)$\backslash$nEND PLOT.

\textcolor{blue}{Edited ChatGPT's answer}: Based on the information given, we can use the angle sum property of a triangle \textcolor{green}{and Congruence of Triangles - SSS} to find the value of angle CBD. In triangle ABC, the sum of the interior angles is 180 degrees: Angle CBA + Angle ACB + Angle BAC = 180 degrees Substituting the given values: 88 degrees + 53 degrees + Angle BAC = 180 degrees Simplifying the equation: 141 degrees + Angle BAC = 180 degrees Subtracting 141 degrees from both sides: Angle BAC = 180 degrees - 141 degrees Angle BAC = 39 degrees Now, in triangle BCD, the sum of the interior angles is also 180 degrees: Angle CBD + Angle BCD + Angle BDC = 180 degrees. \textcolor{green}{According to the Congruence of Triangles - SSS, AB = CD, AC = BD, BC = BC, hence ABC and DCB are congruent. Hence, angle ABC = angle BCD = 88} Substituting the known values: x degrees + \textcolor{red}{\st{90}} \textcolor{green}{88} degrees + 39 degrees = 180 degrees Simplifying the equation: x degrees + \textcolor{red}{\st{129}} \textcolor{green}{127} degrees = 180 degrees Subtracting \textcolor{red}{\st{129}} \textcolor{green}{127} degrees from both sides: x degrees = 180 degrees - \textcolor{red}{\st{129}} \textcolor{green}{127} degrees x degrees = \textcolor{red}{\st{51}} \textcolor{green}{53} degrees Therefore, the value of x in the figure is \textcolor{red}{\st{51}} \textcolor{green}{53} degrees.

% \textcolor{blue}{Edit rate:} 22\%
        \end{minipage} \\

    \end{tabular}
    \caption{Data collecting and annotating process with the edit rate of 12.75\%. \textcolor{red}{Red} text denotes the deleted part of ChatGPT's answer,  \textcolor{green}{green} text denotes the corrected part.}
    \label{tab:post-edit}

% \normalsize
% \raggedright
%     \parbox{7.5cm}{
%     \textcolor{white}{-----------------------------------------------------------}
%     As stated in \Cref{subsec:curri}, ChatGPT's responses undergo post-generation editing to enhance their quality. The editing process serves the purpose of addressing one or more of the following issues: missing information, incorrect calculations, or unnecessary details.}
    
\end{table*}

    

==> gpt2.tex <==
\section{Nonsensical questions generated by GPT-2 fine-tuned model} 
Many questions generated by GPT-2 contains non alphabetical tokens, and most questions generated are "combination of words" instead of actually meaningful questions. We provide some examples in \Cref{tab:gpt2-trash}. 

\begin{table*}[b]

\label{appdx:nonsense-gpt2}
\centering
\small
\begin{tabular}{p{7cm}|p{5.5cm}}
    \toprule
     Context  & Generated question \\
     \midrule 
     At the stop 8 more people got on the train. Initially, there were 11 people on the train. &  @@
 Is there a limit on the number of people on the bus? \\ 
    \midrule
    Randy uses 36 blocks to build a tower. If he had 59 blocks & ia is he planning on building 6 blocks of blocks? \\
    \midrule
    Matthew had 23 crackers. He has 11 crackers left after he gave equal numbers of crackers to his 2 friends. &  
    ????? \\
    \midrule
    At the arcade Dave had won 14 tickets and lost 2 tickets. If he used 10 to buy some toys & 
    $\sim\sim$ How many more tickets did Dave win? \\
    \midrule
    Nell collects baseball cards. She had 573 cards. She gave 195 cards to John and yet some more to Jeff. Now she has 210 cards left. & ers asked the most. \\
    \bottomrule
\end{tabular}
\caption{Generated questions with errors of GPT-2}
\label{tab:gpt2-trash}


\end{table*}
